GG-SSMs: Graph-Generating State Space Models

State Space Models (SSMs) are powerful tools for modeling sequential data in computer vision and time series analysis domains. However, traditional SSMs are limited by fixed, one-dimensional sequential processing, which restricts their ability to model non-local interactions in high-dimensional data. While methods like Mamba and VMamba introduce selective and flexible scanning strategies, they rely on predetermined paths, which fails to efficiently capture complex dependencies. We introduce Graph-Generating State Space Models (GG-SSMs), a novel framework that overcomes these limitations by dynamically constructing graphs based on feature relationships. Using Chazelle's Minimum Spanning Tree algorithm, GG-SSMs adapt to the inherent data structure, enabling robust feature propagation across dynamically generated graphs and efficiently modeling complex dependencies. We validate GG-SSMs on 11 diverse datasets, including event-based eye-tracking, ImageNet classification, optical flow estimation, and six time series datasets. GG-SSMs achieve state-of-the-art performance across all tasks, surpassing existing methods by significant margins. Specifically, GG-SSM attains a top-1 accuracy of 84.9% on ImageNet, outperforming prior SSMs by 1%, reducing the KITTI-15 error rate to 2.77%, and improving eye-tracking detection rates by up to 0.33% with fewer parameters. These results demonstrate that dynamic scanning based on feature relationships significantly improves SSMs' representational power and efficiency, offering a versatile tool for various applications in computer vision and beyond.

==> figures/diagrams/architectures.tex <==
\tikzstyle{every node}=[font=\footnotesize]

\begin{tikzpicture}[>=stealth, xscale=1.0]
\def\l{0.2cm}
\def\r{0.25cm}
\def\w{1.6cm}
\def\h{0.5cm}
\def\dy{0.2cm}
\def\dx{0.5cm}

\def\ws{0.35cm}
\def\hs{\ws}

\tikzstyle{box1}=[
	fill = matlab1!20!white,
	fill opacity = 1.0,
	draw = matlab1,
	draw opacity = 1,
	text opacity = 1,
	minimum width = \w,
	minimum height = \h,
	anchor = center,
	inner sep = 3pt,
	outer sep = 0pt,
	]
	
\tikzstyle{box2}=[
	box1,
	fill = matlab2!20!white,
	draw = matlab2
	]
	
\tikzstyle{box3}=[
	box1,
	fill = matlab3,
	draw = matlab3
	]

\tikzstyle{boxnone}=[
	box1,
	draw=none,
	fill=none
	]	

\tikzstyle{boxno}=[
	box1,
	draw=none,
	fill=none,
	minimum width = 0pt,
	minimum height = 0pt,
	inner sep = 0pt,
	]	
	
\node (add) [boxno] {\tiny\!\large$\bigoplus$\tiny\!};
\node (lin) [box1, below=\dy of add] {Linear};
\node (mul) [boxno, below=\dy of lin] {\tiny\!\large$\bigotimes$\tiny\!};
\node (empty) [boxnone, below=\dy of mul] {};
\node (s6) [box2, below=\dy of empty] {S6};
\node (silu)  [box1, below=\dy of s6] {SiLU};
\node (dw)  [box1, below=\dy of silu] {DWConv1};
\node (lin2)  [box1, below=\dy of dw] {Linear};
\node (rms)  [box1, below=2*\dy of lin2] {RMSNorm};
 
\node (silu2) [box1, right=\dx of silu] {SiLU};
\node (lin3) [box1, right=\dx of lin2] {Linear};

\draw [->] (add) -- ([yshift=2*\dy]add.north);
\draw [->] (rms) -- coordinate [midway] (rmslin2) (lin2);
\draw [->] (lin2) -- (dw);
\draw [->] (dw) -- (silu);
\draw [->] (silu) -- (s6);
\draw [->] (s6) -- (mul);
\draw [->] (mul) -- (lin);
\draw [->] (lin) -- (add);
\draw [->] (rmslin2) -| (lin3);
\draw [->] (lin3) -- (silu2);
\draw [->] (silu2) |- (mul);
\draw [->] ([yshift=-2*\dy]rms.south) -- coordinate [midway] (rmsbelow) (rms);
\draw [->] (rmsbelow) -- ([xshift=-1.3cm]rmsbelow.west) |- (add);

\path ([xshift=-1.3cm]rmsbelow.west) -| coordinate [pos=0.25] (middle)  (lin3.east);
\node (text1) [below=0.5cm of middle] {(a) Mamba Architecture} ;

\node (Xadd) [boxno, right = 5cm of add] {\tiny\!\large$\bigoplus$\tiny\!};
\node (Xlin) [box1, below=\dy of Xadd] {Linear};
\node (Xmul) [boxno, below=\dy of Xlin] {\tiny\!\large$\bigotimes$\tiny\!};
\node (Xempty) [box1, below=\dy of Xmul] {LN};
\node (Xs6) [box2, below=\dy of Xempty] {SS2D};
\node (Xsilu)  [box1, below=\dy of Xs6] {SiLU};
\node (Xdw)  [box1, below=\dy of Xsilu] {DWConv};
\node (Xlin2)  [box1, below=\dy of Xdw] {Linear};
\node (Xrms)  [box1, below=2*\dy of Xlin2] {LN};
 
\node (Xsilu2) [box1, right=\dx of Xsilu] {SiLU};
\node (Xlin3) [box1, right=\dx of Xlin2] {Linear};

\draw [->] (Xadd) -- ([yshift=2*\dy]Xadd.north);
\draw [->] (Xrms) -- coordinate [midway] (Xrmslin2) (Xlin2);
\draw [->] (Xlin2) -- (Xdw);
\draw [->] (Xdw) -- (Xsilu);
\draw [->] (Xsilu) -- (Xs6);
\draw [->] (Xs6) -- (Xempty);
\draw [->] (Xempty) -- (Xmul);
\draw [->] (Xmul) -- (Xlin);
\draw [->] (Xlin) -- (Xadd);
\draw [->] (Xrmslin2) -| (Xlin3);
\draw [->] (Xlin3) -- (Xsilu2);
\draw [->] (Xsilu2) |- (Xmul);
\draw [->] ([yshift=-2*\dy]Xrms.south) -- coordinate [midway] (Xrmsbelow) (Xrms);
\draw [->] (Xrmsbelow) -- ([xshift=-1.3cm]Xrmsbelow.west) |- (Xadd);

\draw [red, dashed] ([xshift=-0.2cm, yshift=0.5cm]Xsilu2.north west) rectangle ([xshift=0.2cm]Xlin3.south east |- Xrmsbelow);
\node [below = 0.3cm of Xlin3, align =center, text width = \w, red]  {Multiplicative \\ Branch};

\path ([xshift=-1.3cm]Xrmsbelow.west) -| coordinate [pos=0.25] (Xmiddle)  (Xlin3.east);
\node at (text1-|Xmiddle) {(b) The VMamba Architecture};

\def\dy{0.4cm}

% First Block (FFN block)
\node (Yadd) [boxno, right = 5cm of Xadd] {\tiny\!\large$\bigoplus$\tiny\!};
\node (Yffn) [box2, below = \dy of Yadd] {FFN};
\node (Yln) [box1, below=\dy of Yffn] {LN};
\draw [->] (Yadd) -- ([yshift=\dy]Yadd.north);
\draw [->] ([yshift=-2*\dy]Yln.south) -- coordinate [midway] (Ylnbelow) (Yln);
\draw [->] (Ylnbelow) --  ([xshift=-1.3cm]Ylnbelow) coordinate (Ylnbelowleft) |- (Yadd);
\draw [->] (Yln) -- (Yffn);
\draw [->] (Yffn) -- (Yadd);

% Second Block (GG-SSM Block)
\node (Zadd) [boxno, below = 1.38cm of Yln] {\tiny\!\large$\bigoplus$\tiny\!};
\node (Zffn) [box2, below = \dy of Zadd] {\shortstack{GG-SSM \\ Block}}; % Use shortstack for vertical alignment
\node (Zln) [box1, below=\dy of Zffn] {LN};
\draw [->] (Zadd) -- (Yln);
\draw [->] ([yshift=-2*\dy]Zln.south) -- coordinate [midway] (Zlnbelow) (Zln);
\draw [->] (Zlnbelow) --  ([xshift=-1.3cm]Zlnbelow) coordinate (Zlnbelowleft)  |- (Zadd);
\draw [->] (Zln) -- (Zffn);
\draw [->] (Zffn) -- (Zadd);


\node (Alin) [box1, right = 2*\dx of Yffn] {Linear};
\node (Aln) [box1, below = \dy of Alin] {LN};
\node (Asd) [box2, below = \dy of Aln] {GG-SSM};
\node (Asilu) [box1, below = \dy of Asd] {SiLU};
\node (Adw) [box1, below = \dy of Asilu] {DWConv};
\node (Alin2) [box1, below = \dy of Adw] {Linear};
\draw [->] (Alin) -- ([yshift=2*\dy]Alin.north);
\draw [->] (Alin2) -- (Adw);
\draw [->] (Adw) -- (Asilu);
\draw [->] (Asilu) -- (Asd);
\draw [->] (Asd) -- (Aln);
\draw [->] (Aln) -- (Alin);
\draw [->] ([yshift=-2*\dy]Alin2.south) -- (Alin2);

\coordinate (r1) at  ([xshift=-\dx, yshift=\dy]Alin.north west);
\coordinate (r2) at ([xshift=\dx, yshift=-\dy]Alin2.south east);
\draw [densely dashed] (r1) rectangle (r2);
\draw [densely dashed] (Zffn.north east) -- (r1);
\draw [densely dashed] (Zffn.south east) -- (r1 |- r2);

\begin{pgfonlayer}{background}
\draw [lightgray!25!white, fill] ([xshift=-0.5*\dx, yshift=0.5*\dy]Yadd.north-|Ylnbelowleft) coordinate (leftmost) rectangle ([xshift=0.5*\dx, yshift=-\dy]Ylnbelowleft-|Yln.south east) ;
\draw [lightgray!25!white, fill] ([xshift=-0.5*\dx, yshift=0.5*\dy]Zadd.north-|Zlnbelowleft)  rectangle ([xshift=0.5*\dx, yshift=-0.5*\dy]Zlnbelowleft-|Zln.south east) ;
\end{pgfonlayer}

\path (leftmost) -| coordinate [pos=0.25] (text3) (r2);
\node at (text1-|text3) {(c) GG-SSM Architecture};

\end{tikzpicture}%

\tikzstyle{every node}=[font=\normalsize]

